A Physical Model-based Correction for Charge Traps in the Hubble Space Telescope's Wide Field Camera 3 Near-IR Detector and Applications to Transiting Exoplanets and Brown Dwarfs

The Hubble Space Telescope (HST) Wide Field Camera 3 (WFC3) near-IR channel is extensively used in time-resolved observations, especially for transiting exoplanet spectroscopy and brown dwarf and directly imaged exoplanet rotational phase mapping. The ramp effect is the dominant source of systematics in the WFC3 for time-resolved observations, which limits its photometric precision. Current mitigation strategies are based on empirical fits and require additional orbits "to help the telescope reach a thermal equilibrium". We show that the ramp effect profiles can be explained and corrected with high fidelity using charge trapping theories. We also present a model for this process that can be used to predict and to correct charge trap systematics. Our model is based on a very small number of parameters that are intrinsic to the detector. We find that these parameters are very stable between the different datasets, and we provide best-fit values. Our model is tested with more than 120 orbits ($\sim40$ visits) of WFC3 observations and is proved to be able to provide near photon noise limited corrections for observations made with both staring and scanning modes of transiting exoplanets as well as for starting-mode observations of brown dwarfs. After our model correction, the light curve of the first orbit in each visit has the same photometric precision as subsequent orbits, so data from the first orbit need no longer be discarded. Near IR arrays with the same physical characteristics (e.g., JWST/NIRCam) may also benefit from the extension of this model, if similar systematic profiles are observed.

==> fig3.tex <==
% \documentclass{article}

% \usepackage{tikz}
% \usetikzlibrary{shapes.geometric, arrows}
% \begin{document}
\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=2cm, minimum height=1cm,text centered, draw=black, text width=5cm]
\tikzstyle{process} = [rectangle, minimum width=2cm, minimum height=1cm, text centered, draw=black, text width=5cm]
\tikzstyle{decision} = [diamond, minimum width=2cm,  text centered, draw=black, aspect=2.5]
\tikzstyle{arrow} = [thick,->,>=stealth]

\begin{center}
\begin{tikzpicture}[node distance=2cm]
  \node (start) [startstop] {Number of initially trapped charges: $E_0$ };
  \node (exposure) [process, below of=start] {$i^{\mathrm{th}}$ exposure, flux $\flux_i(t)$};
  \node (trap) [process, below of=exposure] {Charge trapping/release\\ $\dfrac{\dd \trapped(t)^+}{\dd t} = \eta\,\flux(t)\,\frac{\ntrapo-\trapped}{\ntrapo}$ $\dfrac{\dd \trapped(t)^-}{\dd t} = - \frac{\trapped(t)}{\tau}$};
  % \node (release) [process, below of=gain] {Electron Releasing $\dfrac{\dd \trapped(t)^-}{\dd t} = - \frac{\trapped(t)}{\tau}$};
  \node (measurement) [startstop, below of=trap, yshift=-0.8cm] {Measured flux\\ $\flux'_i(t) = \flux_i(t) - (\dfrac{\dd \trapped_\mathrm{s}(t)}{\dd t} + \dfrac{\dd \trapped_\mathrm{f}(t)}{\dd t})$};
  \node (nTrapped) [process, right of=trap, xshift=4cm,
  yshift=-1.5cm] {Trapped Electrons\\ $E(t) \mathrel{+}= (\dfrac{\dd
      \trapped(t)^+}{\dd t} + \dfrac{\dd \trapped(t)^-}{\dd t}) \dd t$};
  \node (changeorbit) [decision, above of=nTrapped, yshift=0.3cm] {Next orbit?};
  \node (extraE) [process, above of=changeorbit, yshift=0.3cm] {$E(t) \mathrel{+}= \dtrap$};
  \draw [arrow] (start) -- (exposure);
  \draw [arrow] (exposure) -- (trap);
  \draw [arrow] (trap) -- (measurement);
  \draw [arrow] (trap) |- (nTrapped);
  \draw [arrow] (nTrapped) -- (changeorbit);
  \draw [arrow] (changeorbit) -- node [anchor=west,yshift=.2cm]{yes} (extraE);
  \draw [arrow] (changeorbit) |- node [anchor=east,yshift=-.15cm]{no} (exposure);
  \draw [arrow] (extraE) -| (exposure);
\end{tikzpicture}
\end{center}



% \end{document}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

